Modons on Tidally Synchronised Extrasolar Planets

We investigate modons on tidally synchronised extrasolar planets. Modons are highly dynamic, coherent flow structures composed of a pair of storms with opposite signs of vorticity. They are important because they divert flows on the large-scale; and, powered by the intense irradiation from the host star, they are planetary-scale sized and exhibit quasi-periodic life-cycles -- chaotically moving around the planet, breaking and reforming many times over long durations (e.g. thousands of planet days). Additionally, modons transport and mix planetary-scale patches of hot and cold air around the planet, leading to high-amplitude and quasi-periodic signatures in the disc-averaged temperature flux. Hence, they induce variations of the "hot spot" longitude to either side of the planet's sub-stellar point -- consistent with observations at different epoch. The variability behaviour in our simulations broadly underscores the importance of accurately capturing vortex dynamics in extrasolar planet atmosphere modelling, particularly in understanding current observations.

==> chocros.tex <==
\usepackage{amssymb}
\usepackage{upgreek}
\usepackage{bbm}
\usepackage{dsfont}
\usepackage{sansmath}
\usepackage{mathrsfs}
\usepackage{yfonts}
\usepackage{euscript}

\pdfpagewidth=210 true mm
\pdfpageheight=297 true mm

\def\d{{\rm d}}
\def\D{{\rm D}}
\def\del{\partial}
\def\bfnabla{\mbox{\boldmath{$\nabla$}}}
\def\grad-s{\mbox{\boldmath{$\nabla$}}_{\!\! s}\,}
\def\bfx{{\bf x}}
\def\bfu{{\bf u}}
\def\bfv{{\bf v}}
\def\bfk{{\bf k}}
\def\bfOmega{\mbox{\boldmath{$\Omega$}}}
\def\bfomega{\mbox{\boldmath{$\upomega$}}}
\def\bfeta{\mbox{\boldmath{$\upeta$}}}
\def\bfPsi{\mbox{\boldmath{$\Psi$}}}
\def\bfCalF{\mbox{\boldmath{${\cal F}$}}}
\def\bfCalD{\mbox{\boldmath{${\cal D}$}}}
\def\sub#1{\mbox{\tiny $\mbox{\sc {#1}}$}}
\def\mathbi#1{\textbf{\em #1}}
\def\matrixbf#1{\mbox{\large\textbf{\textsf{#1}}}}
\def\tauN{\tau_{\mbox{\tiny{\sc N}}}}
\def\tauR{\tau_{\mbox{\tiny{\sc R}}}}
\def\tauRB{\tau_{\mbox{\tiny{\sc R20}}}}
\def\LD{L_{\rm{\tiny D}}}
\def\EKE{\!{\it EKE\ }}
\def\APE{\!{\it APE\ }}
\def\scrD{\mathscr{D}}
\def\scrE{\mathscr{E}}
\def\scrL{\mathscr{L}}
\def\scrT{\mathscr{T}}
\def\gsim{\;\rlap{\lower 2.5pt\hbox{$\sim$}}\raise 1.5pt\hbox{$>$}\;}
\def\lsim{\;\rlap{\lower 2.5pt\hbox{$\sim$}}\raise 1.5pt\hbox{$<$}\;}

\def\gsim{\;\rlap{\lower 2.5pt\hbox{$\sim$}}\raise 1.5pt\hbox{$>$}\;}
\def\lsim{\;\rlap{\lower 2.5pt\hbox{$\sim$}}\raise 1.5pt\hbox{$<$}\;}
\def\del{{\partial}}
\def\grad{\mbox{\boldmath{$\nabla$}}}
\def\bfOmega{\mbox{\boldmath{$\Omega$}}}
\def\bfF{\mbox{\boldmath{${\cal F}$}}}
\def\bfzeta{\mbox{\boldmath{$\zeta$}}}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\newcommand{\HDblah}{HD~$\!$209458~$\!$b}
\newcommand{\LR}{$L_{\cal R}$}
\newcommand{\BigO}{${\cal O}$}
\newcommand{\pderiv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\aderiv}[1]{\frac{{\rm D} #1}{{\rm D}t}}
\newcommand{\Del}{\bf \nabla} 
\newcommand{\Div}{\Del\cdot} 

\newcommand{\rem}[1]{{\bf[#1]}}

\usepackage{color}
\definecolor{com_red}{rgb}{.8,.2,0.1}
\definecolor{ins_green}{rgb}{.1,.5,0.1}
\newcommand{\ins}[1]{\textcolor{ins_green}{#1}}

